Search for Heavy Right-Handed Neutrinos at the LHC and Beyond in the Same-Sign Same-Flavor Leptons Final State

In this study we explore the LHC's Run II potential to the discovery of heavy Majorana neutrinos, with luminosities between $30$ and $3000$ fb$^{-1}$ in the $l^{\pm}l^{\pm}j~j$ final state. Given that there exist many models for neutrino mass generation, even within the Type I seesaw framework, we use a simplified model approach and study two simple extensions to the Standard Model, one with a single heavy Majorana neutrino, singlet under the Standard Model gauge group, and a limiting case of the left-right symmetric model. We then extend the analysis to a future hadron collider running at $100$ TeV center of mass energies. This extrapolation in energy allows us to study the relative importance of the resonant production versus gauge boson fusion processes in the study of Majorana neutrinos at hadron colliders. We analyze and propose different search strategies designed to maximize the discovery potential in either the resonant production or the gauge boson fusion modes.

==> Diagrams/WWfusion_N.tex <==
%\documentclass[11pt]{article}
%\usepackage{graphicx}
%\usepackage{amsmath,amssymb,amscd}
%\usepackage{axodraw}
\begin{document}
\pagestyle{empty}
\begin{center}
\begin{picture}(400,200)(0,0)
\SetColor{Red}
\ArrowLine(20,170)(60,170)
\ArrowLine(60,170)(100,180)
\SetColor{Green}
\ArrowLine(20,20)(60,20)
\ArrowLine(60,20)(100,10)
\SetColor{Blue}
\Photon(60,170)(60,120){2}{6}
\Photon(60,20)(60,70){2}{6}
\SetColor{Black}
\Line(60,120)(60,70)
\ArrowLine(100,120)(60,120)
\ArrowLine(100,70)(60,70)
\Text(20,180)[c]{$u$}
\Text(100,190)[c]{$d$}
\Text(20,10)[c]{$u$}
\Text(100,0)[c]{$d$}
\Text(50,145)[c]{$W^+$}
\Text(50,45)[c]{$W^+$}
\Text(50,95)[c]{$N$}
\Text(110,120)[c]{$\ell^+$}
\Text(110,70)[c]{$\ell^{\prime +}$}
\Text(65,200)[c]{(a)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetColor{Red}
\ArrowLine(180,170)(220,170)
\ArrowLine(220,170)(260,180)
\SetColor{Green}
\ArrowLine(180,20)(220,20)
\ArrowLine(220,20)(260,10)
\SetColor{Blue}
\Photon(220,170)(220,120){2}{6}
\Photon(220,20)(220,70){2}{6}
\SetColor{Black}
\Line(220,120)(220,70)
\Line(220,120)(245,95)
\Line(220,70)(245,95)
\ArrowLine(270,120)(245,95)
\ArrowLine(270,70)(245,95)
\Text(180,180)[c]{$u$}
\Text(260,190)[c]{$d$}
\Text(180,10)[c]{$u$}
\Text(260,0)[c]{$d$}
\Text(210,145)[c]{$W^+$}
\Text(210,45)[c]{$W^+$}
\Text(210,95)[c]{$N$}
\Text(280,70)[c]{$\ell^+$}
\Text(280,120)[c]{$\ell^{\prime +}$}
\Text(225,200)[c]{(b)}
\end{picture}
\end{center}
\end{document}

==> Diagrams/schannel_N_2.tex <==
%\documentclass[11pt]{article}
%\usepackage{graphicx}
%\usepackage{amsmath,amssymb,amscd}
%\usepackage{axodraw}
\begin{document}
\pagestyle{empty}
\begin{center}
\begin{picture}(400,300)(0,0)
\SetColor{Red}
\ArrowLine(80,80)(110,50)
\ArrowLine(110,50)(80,20)
\ArrowLine(260,50)(290,80)
\ArrowLine(260,50)(290,20)
\SetColor{Blue}
\Photon(110,50)(170,50){2}{6}
\Photon(200,50)(260,50){2}{6}
\SetColor{Green}
\ArrowLine(170,80)(170,50)
\ArrowLine(200,80)(200,50)
\SetColor{Black}
\Line(170,50)(200,50)
\Text(80,90)[c]{$u$}
\Text(80,10)[c]{$\bar{d}$}
\Text(140,40)[c]{$W^+$}
\Text(230,40)[c]{$W^-$}
\Text(185,40)[c]{$N$}
\Text(170,90)[c]{$\ell^+$}
\Text(200,90)[l]{$\ell^{\prime +}$}
\Text(290,90)[c]{$j_1$}
\Text(290,10)[c]{$j_2$}
\Text(185,0)[c]{(a)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetColor{Red}
\ArrowLine(80,200)(110,170)
\ArrowLine(110,170)(80,140)
\ArrowLine(260,170)(290,200)
\ArrowLine(260,170)(290,140)
\SetColor{Blue}
\Photon(110,170)(170,170){2}{6}
\Photon(200,170)(260,170){2}{6}
\SetColor{Green}
\ArrowLine(170,200)(185,185)
\Line(185,185)(200,170)
%\ArrowLine(170,200)(200,170)
\ArrowLine(200,200)(185,185)
\Line(185,185)(170,170)
\SetColor{Black}
\Line(170,170)(200,170)
\Text(80,210)[c]{$u$}
\Text(80,130)[c]{$\bar{d}$}
\Text(140,160)[c]{$W^+$}
\Text(230,160)[c]{$W^-$}
\Text(185,160)[c]{$N$}
\Text(170,210)[c]{$\ell^+$}
\Text(200,210)[l]{$\ell^{\prime +}$}
\Text(290,210)[c]{$j_1$}
\Text(290,130)[c]{$j_2$}
\Text(185,240)[c]{(b)}
\end{picture}
\end{center}
\end{document} 
